Multimodal Prototypical Networks for Few-shot Learning

Although providing exceptional results for many computer vision tasks, state-of-the-art deep learning algorithms catastrophically struggle in low data scenarios. However, if data in additional modalities exist (e.g. text) this can compensate for the lack of data and improve the classification results. To overcome this data scarcity, we design a cross-modal feature generation framework capable of enriching the low populated embedding space in few-shot scenarios, leveraging data from the auxiliary modality. Specifically, we train a generative model that maps text data into the visual feature space to obtain more reliable prototypes. This allows to exploit data from additional modalities (e.g. text) during training while the ultimate task at test time remains classification with exclusively visual data. We show that in such cases nearest neighbor classification is a viable approach and outperform state-of-the-art single-modal and multimodal few-shot learning methods on the CUB-200 and Oxford-102 datasets.

==> sections/_tsne.tex <==
In this section we provide additional visualizations for the embedding spaces in different few-shot learning scenarios. Therefore, we show visualizations for the embedding space in $k$-way classification problems with $k \in \{5,10,20,50\}$. We use t-SNE for dimensionality reduction. The visualizations are shown in Figures~\ref{fig:tsne1}, \ref{fig:tsne2}, \ref{fig:tsne3} and \ref{fig:tsne4} in which the different colors indicate the class membership. Although the dimensionality is reduced to two for being able to visualize the embedding space we can still see the clusters for different classes. It can be observed that in many cases the multimodal prototypes (triangles) are moved towards the center of the cluster for the particular class compared to the image-only prototypes (crosses).
\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \captionsetup{margin=.4cm}
  \includegraphics[width=\linewidth]{figures/tsne_5way_10.pdf}
  \captionof{figure}{t-SNE graph for 5-way classification showing the image-only prototypes (crosses), updated multimodal prototypes (triangles) and unseen test samples (dots)}
  \label{fig:tsne1}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/tsne_10way_7.pdf}
  \captionsetup{margin=.4cm}
  \captionof{figure}{t-SNE graph for 10-way classification showing the image-only prototypes (crosses), updated multimodal prototypes (triangles) and unseen test samples (dots)}
  \label{fig:tsne2}
  
\end{minipage}
\vspace{1cm}
\end{figure}


\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \captionsetup{margin=.4cm}
  \includegraphics[width=\linewidth]{figures/tsne_20way_3.pdf}
  \captionof{figure}{t-SNE graph for 20-way classification showing the image-only prototypes (crosses), updated multimodal prototypes (triangles) and unseen test samples (dots)}
  \label{fig:tsne3}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \captionsetup{margin=.4cm}
  \includegraphics[width=\linewidth]{figures/tsne_50way_10.pdf}
  \captionof{figure}{t-SNE graph for 50-way classification showing the image-only prototypes (crosses), updated multimodal prototypes (triangles) and unseen test samples (dots)}
  \label{fig:tsne4}
\end{minipage}
\vspace{0.5cm}
\end{figure}

==> sections/background.tex <==
\label{sec:background}

\textbf{GAN:} 
GANs \citep{goodfellow_generative_2014} consist of two adversarial agents that compete with each other during a Minimax game until reaching a Nash equilibrium at convergence of the training phase. 
Specifically, they decompose into two main components. \\
First, a \emph{generator} $G$ aims to produce \emph{fake} image data $i_{fake}$ resembling \emph{real} data. That is $i_{fake} = G(z)$, given a random noise vector $z$, which induces a generator distribution $p_G$. Second, a \emph{discriminator} $D$ that defines a mapping $D: \mathcal{I}\to \left[0,1\right]$ that given an image $i\in I$, outputs a distribution w.r.t. state $s$ (i.e. \emph{fake} or \emph{real}), $p(s\mid i)=D(i)$. To this end, the GAN parameters are obtained by optimization of the loss function $\mathcal{L}\left(.\right)$,

\begin{equation}
\label{stdGANloss}
\mathcal{L}_{GAN}\left(G,D\right)=\mathbb{E}_{I}\left[\log D\left(I\right)\right]+\mathbb{E}_{z}\left[\log D\left(I,G\left(z\right)\right)\right].
\end{equation}
Specifically, training the GAN entails alternating optimization of $D$ and $G$ using stochastic gradient-based descent.
\citep{goodfellow_generative_2014} prove that a global optimium is reached when $p_g = p_{data}$, and under mild conditions  eventually $p_g$ converges to $p_{data}$.\\
\textbf{Conditional GAN:}
Conditional GANs (cGANs)~\citep{DBLP:journals/corr/MirzaO14} constitute an extension of the standard GAN, where the input of the generator as well as discriminator are further tied to a conditional variable containing extra information. That condition variable be an kind of auxiliary information such as a class label \citep{DBLP:journals/corr/MirzaO14}, an attribute vector \citep{yan2016attribute2image} or a semantic description~\citep{reed16_gen}. To this end, the standard loss Eq.~\ref{stdGANloss} changes slightly to

\begin{equation}
\label{cGANloss}
\mathcal{L}_{GAN}\left(G,D\right)=\mathbb{E}_{I}\left[\log D\left(I\mid y \right)\right]+\mathbb{E}_{z}\left[\log D\left(I,G\left(z\mid y\right)\right)\right],
\end{equation}
where the conditional variable is denoted as $y$. Technically, conditioning is commonly achieved by concatenation of variables, although there exist numerous possibilites - see~\citet{KwakZ16a} for some examples.

==> sections/ext_result.tex <==
In this section we provide additional results for the quantitative evaluations of our method in our main paper.
\subsection{Results for multimodal 50-way classification}
We extend Tab. 1 from the main paper which shows the accuracies for 50-way classification in comparison with state-of-the-art multimodal few-shot learning methods and our baselines. While in the paper we only reported the top-5 accuracy, we provide top-1 and top-3 accuracy in addition in Tab.~\ref{tab:results_multimodal}. We can observe the same trends as for the top-5 accuracy. %In almost all cases our method outperforms existing approaches and our baselines in every $n$-shot scenario in all metrics.

\begin{table*}[ht]
    \setlength{\tabcolsep}{5pt}
	\centering{
		\begin{tabular}{lccccccc} \toprule
		Dataset & Method & Metric & 1-shot & 2-shot & 5-shot & 10-shot &20-shot \\ \midrule
		CUB & Pahde et al. \cite{pahdeWACV} & Top-1& 24.90 & 25.17 & 34.66 & 44.00 & 53.70 \\
		&&Top-3& 37.59 & 39.75 & 49.86 & 59.62 & 67.99 \\
		&&Top-5& 57.67 & 59.83 & 73.01 & 78.10 & 84.24 \\
		& Image Only Baseline & Top-1&28.91$\pm$0.18 & 37.52$\pm$0.15 & 47.33$\pm$0.12 & 52.31$\pm$0.12 & \textbf{55.62$\pm$0.14}\\
		&&Top-3& 51.13$\pm$0.22 & 62.23$\pm$0.16 & 72.53$\pm$0.11 & 76.71$\pm$0.09 & 78.87$\pm$0.10\\
		&&Top-5& 62.65$\pm$0.22 & 73.52$\pm$0.15 & 82.44$\pm$0.09 & 85.64$\pm$0.08 & 87.27$\pm$0.08 \\
		& ZSL Baseline  & Top-1& 22.39$\pm$0.18 & 27.15$\pm$0.16 & 32.24$\pm$0.15 &  34.65$\pm$0.13 & 36.42$\pm$0.17\\
		&&Top-3& 45.37$\pm$0.21 & 52.42$\pm$0.18 & 59.09$\pm$0.14 & 61.73$\pm$0.13 & 63.27$\pm$0.15 \\
		&&Top-5& 58.28$\pm$0.22 & 65.62$\pm$0.19 & 71.79$\pm$0.14 & 74.15$\pm$0.11 & 75.32$\pm$0.13 \\
		& Our (Multimodal) &Top-1&  \textbf{34.16$\pm$0.17} & \textbf{41.43$\pm$0.14} & \textbf{48.84$\pm$0.10} & \textbf{53.01$\pm$0.11} & 55.58$\pm$0.14\\
		&&Top-3& \textbf{58.56$\pm$0.19} & \textbf{67.44$\pm$0.13} & \textbf{74.65$\pm$0.09} & \textbf{77.60$\pm$0.09} &  \textbf{79.30$\pm$0.11}\\
		&&Top-5& \textbf{70.39$\pm$0.19} & \textbf{78.62$\pm$0.12} & \textbf{84.32$\pm$0.06} & \textbf{86.23$\pm$0.08} & \textbf{87.47$\pm$0.09} \\\midrule
		Oxford-102 & Pahde et al. \cite{pahdeWACV}
		&Top-1& 43.77 &	61.42	& 72.49 & - & - \\
		&&Top-3& 57.96	&77.68	&82.18 & - & - \\
		&&Top-5& 78.37 & 91.18 & 92.21 & - & - \\
		
		
		& Image Only Baseline & Top-1&  49.39$\pm$0.34 &60.02$\pm$0.27 & 70.24$\pm$0.18 & 74.49$\pm$0.16 & \textbf{76.98$\pm$0.16}\\
		&&Top-3& 74.12$\pm$0.32  & 82.76$\pm$0.21&  89.11$\pm$0.12& 91.34$\pm$0.11 & 92.46$\pm$0.10\\
		&&Top-5& 83.88$\pm$0.27 &  90.27$\pm$0.16 & 94.25$\pm$0.09 & 95.61$\pm$0.08 & 96.21$\pm$0.08 \\
		
		
		
		& ZSL Baseline  & Top-1& 34.99$\pm$0.32  & 39.63$\pm$0.29& 42.92$\pm$0.24 & 44.21$\pm$0.22 & 44.91$\pm$0.21\\
		&&Top-3& 60.90$\pm$0.34 &65.91$\pm$0.30 & 69.89$\pm$0.23 & 71.70$\pm$0.21 & 72.76$\pm$0.20 \\
		&&Top-5& 73.14$\pm$0.31 & 77.63$\pm$0.27 & 81.10$\pm$0.19 & 82.88$\pm$0.18 & 84.00$\pm$0.17 \\
		
		
		
		& Our (Multimodal) &Top-1& \textbf{53.70$\pm$0.30}   & \textbf{62.46$\pm$0.24}& \textbf{71.08$\pm$0.19} & \textbf{74.73$\pm$0.17} &76.77$\pm$0.15\\
		&&Top-3& \textbf{77.71$\pm$0.25}  &\textbf{84.35$\pm$0.18} & \textbf{89.51$\pm$0.11} & \textbf{91.53$\pm$0.11} & \textbf{92.48$\pm$0.10}\\
		&&Top-5& \textbf{86.34$\pm$0.21}& \textbf{91.30$\pm$0.15} & \textbf{94.58$\pm$0.09} & \textbf{95.77$\pm$0.08} & \textbf{96.34$\pm$0.07}\\
		%Oxford-102 & Pahde et al. \cite{pahdeWACV} & 78.37 & 91.18 & 92.21 & - & - \\
		%& Image Only Baseline (Resnet-18+NN) & 84.18$\pm$0.48 &  90.25$\pm$0.20 & 94.18$\pm$0.13 & 95.63$\pm$0.14 & 96.25$\pm$0.10\\
		%& ZSL Baseline (Generated Resnet-18+NN) & 73.35$\pm$0.52 & 77.52$\pm$0.34 & 81.14$\pm$0.25 & 82.95$\pm$0.28 & 83.97$\pm$0.21 \\
		%& Our Method (Multimodal Resnet-18 + NN) & \textbf{86.52$\pm$0.36}& \textbf{91.31$\pm$0.18} & \textbf{94.57$\pm$0.13} & \textbf{95.74$\pm$0.13} & \textbf{96.38$\pm$0.10}\\
		\bottomrule
		\end{tabular}
	}
	\captionsetup{position=above}
	\captionof{table}{50-way classification top-1, top-3 and top-5 accuracies in comparison to other multimodal few-shot learning approaches and our baselines for CUB-200 and Oxford-102 datasets with $n\in\{1,2,5,10,20\}$. The best results are in bold.}
	\label{tab:results_multimodal}
\vspace{-0.5cm}
\end{table*}

\subsection{Results for additional k-way n-shot classification tasks}
To extend the results in Tab. 2 in the main paper, we evaluate our method in additional k-way classification scenarios with $k \in \{5,10,20\}$. For this experiment we compare our full method to the image-only baseline. Further extending Tab. 2 from the main paper, we report top-3 and top-5 accuracy in addition to the top-1 accuracy. The results for different $n$-shot scenarios with $n \in \{1,2,5,10,20\}$ are shown in Tab.~\ref{tab:results_singlemodal}. It can be observed that in the most scenarios our method improves the classification accuracies and decreases the variance. However, the more visual data is available (higher $n$), the less impact have the generated features.
\begin{table*}[h!]
    \setlength{\tabcolsep}{6pt}
	\centering{
		\begin{tabular}{llcccccc} \toprule
		Task & Method  & Metric & 1-shot & 2-shot & 5-shot & 10-shot & 20-shot\\ \midrule
            5-way & Image Only Baseline& Top-1 & 68.85$\pm$0.86 & 79.99$\pm$0.66 & 83.93$\pm$0.57& 86.95$\pm$0.49 &\textbf{87.78$\pm$0.48}\\
            
            && Top-3 & 94.71$\pm$0.34 &97.80$\pm$0.16 & 98.39$\pm$0.12 &98.91$\pm$0.09&98.95$\pm$0.09\\
            && Top-5 & - & - & - &-&-\\
            
            & Our (Multimodal)&Top-1 &  \textbf{75.01 $\pm$ 0.81} & \textbf{80.90$\pm$0.64}& \textbf{85.30 $\pm$ 0.54} & \textbf{86.96$\pm$0.48}&87.67$\pm$0.51
            \\
                        && Top-3 & \textbf{96.83$\pm$0.25} & \textbf{98.06$\pm$0.14}& \textbf{98.65$\pm$0.11} & \textbf{98.94$\pm$0.08}&\textbf{99.02$\pm$0.09}\\
            && Top-5 & - &- & - &-&-\\\midrule
            
            
            
            
            
            10-way & Image Only Baseline& Top-1 & 59.34$\pm$0.76 & 68.25$\pm$0.65 & 75.72$\pm$0.61 &78.12$\pm$0.60&\textbf{79.68$\pm$0.85}\\
                        && Top-3 & 86.19$\pm$0.51 & 91.67$\pm$0.33 & 94.66$\pm$0.25& \textbf{95.65$\pm$0.24} &\textbf{95.99$\pm$0.31}\\
            && Top-5 & 94.50$\pm$0.29 & 97.20$\pm$0.15 & 98.24$\pm$0.11& 98.55$\pm$0.11 &\textbf{98.63$\pm$0.14}\\
            
            & Our (Multimodal)&Top-1 & \textbf{62.25$\pm$0.73}  & \textbf{69.71$\pm$0.63}  & \textbf{76.02}$\pm$0.62& 78.12$\pm$0.64 &79.29$\pm$0.82\\
                        && Top-3 & \textbf{88.41$\pm$0.45} & \textbf{92.78$\pm$0.28} & \textbf{94.88$\pm$0.23}& 95.55$\pm$0.25 &95.89$\pm$0.31\\
            && Top-5 & \textbf{95.80$\pm$0.25} & \textbf{97.57$\pm$0.14} & \textbf{98.32$\pm$0.11} & \textbf{98.57$\pm$0.11} &98.62$\pm$0.12\\
            \midrule
            
            
            20-way & Image Only Baseline& Top-1 & 46.55$\pm$0.40 & 55.94$\pm$0.36& 64.64$\pm$0.39 & \textbf{68.21$\pm$0.43} &\textbf{69.97$\pm$0.47}\\
                        && Top-3 & 73.60$\pm$0.38 & 81.94$\pm$0.28 & 87.93$\pm$0.23 &89.66$\pm$0.22&\textbf{90.55$\pm$0.26}\\
            && Top-5 & 84.37$\pm$0.30 & 90.56$\pm$0.19 & 94.06$\pm$0.14 &94.96$\pm$0.14&\textbf{95.49$\pm$0.15}\\
            
            & Our (Multimodal)&Top-1 & \textbf{48.23$\pm$0.40 } &\textbf{57.02$\pm$0.36}& \textbf{64.94$\pm$0.38} &68.08$\pm$0.43&69.62$\pm$0.44\\
                        && Top-3 &\textbf{75.31$\pm$0.36} & \textbf{82.90$\pm$0.27}& \textbf{88.31$\pm$0.22}&\textbf{89.75$\pm$0.21}&90.51$\pm$0.24\\
            && Top-5 & \textbf{85.65$\pm$0.29} & \textbf{91.23$\pm$0.18} & \textbf{94.27$\pm$0.14}&\textbf{95.02$\pm$0.13}&95.42$\pm$0.14 \\
            \bottomrule
		\end{tabular}
	}
	\captionsetup{position=above}
	\captionof{table}{Top-1, top-3 and top-5 accuracies for different $k$-way classification tasks on the CUB-200 dataset of our approach compared to our image-only baseline. We report the average accuracy of 600 randomly sampled few-shot episodes including 95\% confidence intervals. The best results are in bold.}
	\label{tab:results_singlemodal}
	

\end{table*}





==> sections/introduction_old.tex <==

The lack of data generally results in inferior model accuracy. Particularly fine-grained categorization tasks necessitate a larger amount of training samples as the distances between different classes are small. Therefore, the classification model has to obtain a basic understanding of parts and attributes of the particular domain, such that considerably many training samples are necessary.  
This stands in stark contrast to the human ability to
% learning is insusceptible, Furthermore, the requirement for large amounts of training data is in stark contrast to human learning, which can 
quickly learn from only few instances. 
% This makes alternative learning approaches that require less training data an attractive research topic. 
As a consequence, research in the domain of few-shot learning, i.e. learning and generalizing from only few training samples, has gained more and more interest (e.g. \citet{vinyals_matching_2016, bertinetto_learning_2016, ravi_optimization_2017, hariharan_low-shot_2017, snell_prototypical_2017}). 
However, research has mainly focused on utilizing only one data modality, mostly images, so far. 
% Overcoming this limitation and 
By including data from additional modalities (e.g. textual descriptions) we can overcome limitations in the low data regime, resulting in improved model performance. Specifically, the second modality (i.e. textual description) can provide additional weak supervision for the classification training. In the context of fine-grained visual categorization, this weak supervision can provide valuable information about parts and attributes of the categories. For example if the fine-grained classification task is to classify different bird species, the description can contain information about the shape of the beak or the color of the wings. In turn, this information can be beneficial to train visual classifiers in the low data regime, because it can specifically guide the model to discriminative regions of the image. Having this additional information allows to reduce the necessity of labeled samples at the expense of additional per-sample annotation (i.e. textual description).
Our key assumption is that incorporating multimodal data in training (i.e. images and fine-grained descriptions thereof) forces the model to identify highly discriminative features \textit{across modalities}, facilitating the training of classification models for fine-grained recognition tasks in few-shot scenarios.
% (e.g. parts in the image and textual attributes in the description).
Specifically, pursuing multimodality suggests that novel classes with low training data in one modality can benefit from previously learned features. 
\begin{figure*}[t!]
	\centering
  \includegraphics[width=0.9\textwidth]{figures/taskFigure.jpg}
	\caption{Learn classifier from dataset extended by hallucinated data conditioned on text}
	\label{fig:taskFigure}
\end{figure*}
%This would enable them to be characterized more efficiently and accurately, resulting in improved performance in the few-shot learning setting (cf. \citep{elhoseiny_link_2017}). 
%Here, we realize this assumption and extend few-shot learning to deal with multimodal data. In this paper, we target multimodal few-shot learning problem in a meta-learning fashion. For that, we split the classes into \emph{base} classes for which many samples exist and \emph{novel} classes with just a few samples, and the data from base classes is used to learn meaningful representations in order to perform few-shot learning on novel classes. This scenario is multi-modal in training and single-modal in testing, and the task is to utilize multimodal data of training set, to learn explicit visual classifiers for novel classes. To that end, the training samples are tuples consisting of an image and a textual description and in test time, however, the model is tested only with the image data from novel classes (see Figure 1).
In this regard, we propose to extend few-shot learning to incorporate multimodality in a meta-learning fashion. Typical few-shot learning tasks split the data into \emph{base} classes that contain many training samples and \emph{novel} classes for which the availability of training data is limited to only a few samples per category (e.g. \citet{hariharan_low-shot_2017}).  %Specifically, we target a scenario for multimodal few-shot learning that mimics situations that arise in practice. 
Specifically, we assume a scenario that is multimodal during training (i.e. images and texts) and single-modal during testing time (i.e. images). This comes with the associated task to utilize multimodal data in base classes and to learn explicit visual classifiers for novel classes. This scenario for multimodal few-shot learning mimics situations that often arise in practice.
In such cases, cross-modal data hallucination is a viable solution as it facilitates few-shot learning by hallucinating images conditioned on fine-grained textual descriptions, and thus solving the scarce data problem. Intuitively, the hallucinator generates images focusing on the previously learned discriminative features. In this regard, Generative Adversarial Networks (GANs) have proven to be very effective for cross-modal sample generation. GANs~\citep{goodfellow_generative_2014} are deep networks mainly applied for unsupervised tasks and commonly used to generate data (e.g. images). The supervisory information in a GAN is indirectly provided within the frame of an adversarial game between two independent networks: a generator ($G$) and a discriminator ($D$). During training, $G$ generates new data and $D$ tries to understand whether its input is real, i.e. whether it is a training image or if it was generated by $G$. This competition between $G$ and $D$ is helpful in boosting the accuracy of both $G$ and $D$. At testing time, only $G$ is used to generate new data. Specifically, the {\em text-conditioned} GANs (e.g. \citep{reed16_gen, zhang_stackgan++:_2017}) that we use in our approach, take as input a text and generate an image, accordingly. Training the text-conditioned GAN allows for the generation of a potentially infinite number of visual samples given some fine-grained textual descriptions. However, the challenge is to pick adequate samples out of the pool of generated samples that allow for building a better classifier within the few-shot scenario. Such subset of images should not only be realistic but in particular class-discriminative. To this end, we follow the \emph{self-paced strategy} and select a subset of images corresponding to the ones in which the generator is most confident about their ``reality'' and the discriminator is the most confident about their ``class-discriminativeness''. 

==> sections/ret.tex <==
As an additional experiment we use the generated feature vectors to retrieve the closest unseen test images in the 5-way 1-shot learning scenario. The feature vectors are generated conditioned on the textual descriptions of the training images. We calculate the distance between feature vectors using the cosine distance measure. The retrieval results for some randomly selected feature vectors are shown in Fig.~\ref{fig:retrieval}. This shows the effectiveness of the text-conditional feature generator. It can be seen that most of the retrieved images are from the correct class. Thus, the generated feature vector is close to unseen test images of the same class, facilitating classification with a nearest neighbor approach.

\begin{figure}[t!]
	\centering
  \includegraphics[width=\textwidth]{figures/retrievalResults.pdf}
	\caption{Retrieval Results for generated feature vectors in a 5-way classification task: The left column shows the textual description (one random caption out of the ten available descriptions per training image), in the middle are the top-5 retrieved unseen test images and in the right column is the training image for the particular class. The color of the surrounding box indicates whether the retrieved test image is from the correct class (green) or a wrong class (red).}
	\label{fig:retrieval}
\end{figure}

